An Asynchronous Distributed Framework for Large-scale Learning Based on Parameter Exchanges

In many distributed learning problems, the heterogeneous loading of computing machines may harm the overall performance of synchronous strategies. In this paper, we propose an effective asynchronous distributed framework for the minimization of a sum of smooth functions, where each machine performs iterations in parallel on its local function and updates a shared parameter asynchronously. In this way, all machines can continuously work even though they do not have the latest version of the shared parameter. We prove the convergence of the consistency of this general distributed asynchronous method for gradient iterations then show its efficiency on the matrix factorization problem for recommender systems and on binary classification.

==> experiments_mf.tex <==

\section{Experimental Results for Matrix Factorization}
\label{sec:Exp_MF}
We conducted a number of experiments to empirically validate the proposed asynchronous framework on matrix factorization for recommendation where the recommendation matrix is split into $M$ rows as in Problem~\eqref{eqn:pb-split}.

\subsection{Experimental Settings:}

\textbf{Datasets:} We performed experiments on  Movielens-10M (ML-10M)\footnote{http://grouplens.org/datasets/movielens/} and the Netflix Collection\footnote{http://www.netflixprize.com/} that are two popular corpora in collaborative filtering. 

\hspace{-5mm}\textbf{Baselines:}To validate the asynchronous distributed algorithm described in the previous section, we compare the following four strategies:
\begin{itemize}
\item The proposed approach (${\AGDMF}$) ,
\item The asynchronous distributed ADMM approach (\texttt{AD-ADMM})  \cite{Tsung15},
\item Two distributed algorithms specifically proposed for matrix factorization {\ASGD} \cite{makari2015shared} and {\DSGD} \cite{gemulla2011large} (Section \ref{sec:MF}).
\end{itemize}

\hspace{-5mm}\textbf{Platform:} The distributed framework we considered was implemented using PySpark version 1.5.1. by connecting 7 servers with different computational power. 

\hspace{-5mm}\textbf{Hyper-Parameters:} Various free parameters of {\SGO} such as learning rate ($\gamma$), regularization parameter ($\lambda$) and number of latent factors ($K$) were set following \cite{chin2015learning}, \cite{yu2014distributed}. These values as well as the datasets characteristics  are listed in Table \ref{tab:dataset_properties}.

\begin{table}[h!]
\caption{Characteristics of Datasets used in our experiments. $|\mathcal U|$ and $|\mathcal I|$ denote respectively the number of users and items.} %$\alpha$, $\lambda$ and $K$ are respectively the learning rate, the regularisation hyperparameter and the number of latent factors.}
\label{tab:dataset_properties}
\tabcolsep=0.08cm
\centering
\resizebox{\textwidth}{!}{
  \begin{tabular}{ l c c c c c c c c}
  \hline
  Dataset & $|\mathcal U|$ & $|\mathcal I|$ & $\gamma$ & $\lambda$ & $K$ &  training size &  test size & sparsity\\
  \hline
  
    ML-10M & 71567 & 10681 & 0.005 & 0.05 & 100 &  9301274 & 698780 & 98.7 \%\\
  
    NetFlix (NF) & 480189 & 17770 & 0.005 & 0.05 & 40 &  99072112 & 1408395 & 99.8 \%\\

    NF-Subset & 28978 & 1821 & 0.005 & 0.05 & 40 &  3255352 & 100478 & 93.7 \%\\
    
  
  
  \hline
   
\end{tabular}
}
\end{table}


\subsection{Evaluation of Convergence Time}

We begin our experiments by comparing the evolution of the loss function of Eq.~\eqref{eqn:pb} with respect to time until convergence. The convergence points are shown as names of the algorithms vertically (we stopped ASGD after 20 hours on the NF dataset). Figure \ref{fig:RMSE_Curve} depicts this evolution for ML-10M and NF datasets using 10 and 15 cores respectively. Synchronization based approaches ({\ASGD} and {\DSGD}) aggregate all the information at each epoch and thus begin to converge more sharply at the beginning. However, with these approaches, when the fastest machines finish their computations, they have to wait for slower machines; thus, they require much more time to converge than the asynchronous methods (\texttt{AD-ADMM} and ${\AGDMF}$). 
Finally, it comes out that ${\AGDMF}$ converges faster than the other algorithms on both datasets. This is mainly due to the fact that ${\AGDMF}$ does not obey to any delay mechanism as in \texttt{AD-ADMM} for instance.

\subsection{Computation and Communication Trade-off }

We performed another set of experiments aimed at measuring the effect of number of cores on performance of the proposed approach and the baselines. Figure \ref{fig:AverageTimeVsCores} depicts this effect by showing the evolution of time per epoch of the SGD method used in ${\AGDMF}$, \texttt{ASGD}, \texttt{DSGD} and \texttt{AD-ADMM} with respect to increasing number of machines. From these experiments, it comes out that for all approaches the time per epoch of the SGD method decreases as the number of machines increases. 

But after a certain number of machines (10 in both experiments), the time per epoch of some approaches begin to be affected as the communication cost takes over the computation time. The approach that is the most affected by this is \texttt{DSGD}, as synchronizations in this case are done after each sub-epoch. We can also see that even though the per epoch speedup is best for \texttt{ASGD}, it requires a much higher number of epochs to converge as compared to ${\AGDMF}$ and \texttt{DSGD}. 

\iffalse
Finally, it is to be noted that Spark does not provide functionality for inter machine communication and in our implementation we saved the broadcasted parameters for the asynchronous approaches using a distributed storage (HDFS). There exist other frameworks (e.g. Message Passing Interface - MPI) that allow cores to broadcast their parameters directly to other ones and the communication overhead could be significantly reduced in this case.
\fi


\setcounter{figure}{2}
\begin{figure*}[t]
\centering
\begin{subfigure}[b]{0.5\linewidth}
  \centering
  \begin{tikzpicture}
  \begin{axis}[ 
	width=\textwidth,
	height=\textwidth,
 %xmajorgrids, 
 ymajorgrids, 
yminorgrids,
   compat=newest, 
   xmin=5, xmax=21,
   ymin=110, 
   ymax=115,
  %  xtick={0.,20, 40, 60,80},
  %  ytick={0.8, 0.9, 1},
   xlabel=\text{\small time (hour.)},
    ylabel=\text{\small Loss function},
    legend style={font=\tiny},
extra x ticks={19,22,20.8,25},
extra x tick labels={\color{red} \footnotesize  \textbf{$\AGDMF$}, \color{green!50!black} \footnotesize  \textbf{ASGD},  \color{cyan!80!black} \footnotesize  \textbf{DSGD}, \color{magenta!80!black} \footnotesize  \textbf{AD-ADMM},},
extra x tick style={grid=major, tick label style={yshift=0.45cm,rotate=90,anchor=west}},
  ]  

\addplot [ 
 color=red,  
%smooth,
 line width=0.8pt, 
 mark size=1.9pt, 
 mark=diamond*,
 mark options={solid,fill=red,draw=red}, 
 ] 
coordinates {
(0.00,321.84)(1.60,129.39)(3.19,119.13)(4.79,116.01)(6.39,114.37)(7.99,113.31)(9.58,112.56)(11.18,112.00)(12.78,111.55)(14.38,111.21)(15.97,110.92)(17.57,110.67)(19.17,110.40)
};
\addlegendentry{$\AGDMF$}

\addplot [ 
 color=green!50!black,  
 %dashed,
%smooth,
 line width=0.8pt, 
 mark size=1.1pt, 
 mark=square*,
 mark options={solid,fill=green!50!black,draw=green!50!black}, 
 ] 
coordinates {

(0.00,322.18)(1.59,123.99)(3.18,117.48)(4.77,115.02)(6.36,113.73)(7.95,112.89)(9.54,112.28)(11.13,111.81)(12.72,111.44)(14.31,111.14)(15.90,110.90)(17.49,110.70)(19.08,110.53)(20.67,110.38)

};
\addlegendentry{ASGD}

\addplot [ 
 color=cyan!80!black,  
% dashed,
 smooth,
 line width=0.8pt, 
 mark size=1.1pt, 
 mark=*,
 mark options={solid,fill=cyan!80!black,draw=cyan!80!black}, 
 ]  coordinates {
(0.00,284.20)(2.08,120.02)(4.17,115.40)(6.25,113.59)(8.33,112.64)(10.42,111.96)(12.50,111.50)(14.58,111.15)(16.67,110.82)(18.75,110.60)(20.83,110.45)(22.92,110.41)

};
\addlegendentry{DSGD}

\addplot [ 
 color=magenta!80!black,  
 smooth,
 line width=0.8pt, 
 mark size=1.8pt, 
 mark=star,
 %mark options={fill=cyan!50!black}, 
 ]  coordinates {
(1.66,133.73)(3.31,120.46)(4.97,116.70)(6.63,114.85)(8.28,113.68)(9.94,112.88)(11.60,112.28)(13.26,111.84)(14.91,111.48)(16.57,111.19)(18.23,110.93)(19.88,110.69)(21.54,110.52)

};
\addlegendentry{AD-ADMM}
{font=\fontsize{4}{5}\selectfont}

\end{axis}
\end{tikzpicture}
  \caption{(a) NF}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}[b]{0.5\linewidth}
  \centering
  \begin{tikzpicture}
  \begin{axis}[ 
	width=\textwidth,
	height=\textwidth,
   compat=newest, 
   %xmajorgrids,
   ymajorgrids,
   xmin=60, xmax=325,
     ymin=95, 
     ymax=110,
    %xtick={0.,50, 100, 150,200},
    %ytick={0.8, 0.9, 1, 1.1, 1.2},
   xlabel=\text{\small time (min.)},
    ylabel=\text{\small Loss Function},
    legend style={font=\tiny},
extra x ticks={210,308.33,266.67,250.83},
extra x tick labels={\color{red} \footnotesize  \textbf{$\AGDMF$}, \color{green!50!black} \footnotesize  \textbf{ASGD},  \color{cyan!80!black} \footnotesize  \textbf{DSGD}, \color{magenta!80!black} \footnotesize  \textbf{AD-ADMM},},
extra x tick style={grid=major, tick label style={yshift=1.5cm,rotate=90,anchor=west}},
  ]  

\addplot [ 
 color=red,  
%smooth,
 line width=0.8pt, 
 mark size=1.9pt, 
 mark=diamond*,
 mark options={solid,fill=red,draw=red}, 
 ]  coordinates {
 
(0,621.97)(15,135.34)(30,115.73)(45,109.89)(60,106.69)(75,104.63)(90,103.14)(105,102.02)(120,101.14)(135,100.43)(150,99.8)(165,99.29)(180,98.84)(195,98.39)(210,97.68)


};
\addlegendentry{$\AGDMF$}

\addplot [ 
 color=green!50!black,  
 %dashed,
%smooth,
 line width=0.8pt, 
 mark size=1.1pt, 
 mark=square*,
 mark options={solid,fill=green!50!black,draw=green!50!black}, 
 ] coordinates {
(0.00, 627.18)(15.42, 131.33)(30.83, 116.2)(46.25, 110.49)(61.67, 107.27)(77.08, 105.15)(92.50, 103.63)(107.92, 102.48)(123.33, 101.57)(138.75, 100.82)(154.17, 100.21)(169.58, 99.68)(185.00, 99.23)(200.42, 98.84)(215.83, 98.48)(231.25, 98.18)(246.67, 97.91)(262.08, 97.67)(277.50, 97.45)(292.92, 97.26)(308.33, 97.08)
};
\addlegendentry{ASGD}

\addplot [ 
 color=cyan!80!black,  
% dashed,
 smooth,
 line width=0.8pt, 
 mark size=1.1pt, 
 mark=*,
 mark options={solid,fill=cyan!80!black,draw=cyan!80!black}, 
 ] coordinates {
(0.00,517.82)(26.67,115.25)(53.33,107.39)(80.00,104.16)(106.67,102.41)(133.33,101.23)(160.00,100.34)(186.67,99.64)(213.33,99.1)(240.00,98.55)(266.67,98.33)};
\addlegendentry{DSGD}


\addplot [ 
 color=magenta!80!black,  
 smooth,
 line width=0.8pt, 
 mark size=1.8pt, 
 mark=star,
 %mark options={fill=cyan!50!black}, 
 ]  coordinates {
(0.00,621.79)(17.92,136.25)(35.83,116.48)(53.75,110.38)(71.67,107.08)(89.58,104.93)(107.50,103.39)(125.42,102.23)(143.33,101.27)(161.25,100.5)(179.17,99.88)(197.08,99.34)(215.00,98.87)(232.92,98.42)(250.83,98.01)};
\addlegendentry{AD-ADMM}

{font=\fontsize{4}{5}\selectfont}

\end{axis}

\end{tikzpicture}
  
 \label{fig:sub2}
\caption{(b) ML-10M}
\end{subfigure}

\caption{Test RMSE curves with respect to time for {$\AGDMF$}, \texttt{AD-ADMM}, {\ASGD},  and {\DSGD} on NetFlix (a), and ML-10M (b) Datasets}
\label{fig:RMSE_Curve}
\end{figure*}

\setcounter{figure}{3}
\begin{figure*}
\begin{subfigure}[b]{0.5\linewidth}
  \centering
  \begin{tikzpicture}
  \begin{axis}[ 
	width=\textwidth,
	height=\textwidth,
 xmajorgrids, 
 ymajorgrids, 
yminorgrids,
   compat=newest, 
   xmin=3, xmax=22,
   ymin=25, 
   ymax=100,
    xtick={5.,10, 15, 20},
    ytick={25, 50, 75, 100},
    xlabel=\text{\small Number of Cores },
    ylabel=\text{\small Time Per Epoch (sec)},
    legend style={font=\tiny},
%extra x ticks={41.8,64,60,75},
%extra x tick labels={\color{red} \footnotesize  \textbf{Async}, \color{green!50!black} \footnotesize  \textbf{ASGD},  \color{cyan!80!black} \footnotesize  \textbf{DSGD}, \color{magenta!80!black} \footnotesize  \textbf{AsyncWithDelay},},
%extra x tick style={grid=major, tick label style={rotate=90,anchor=west}},
  ]  

\addplot [ 
 color=red,  
%smooth,
 line width=0.8pt, 
 mark size=1.9pt, 
 mark=diamond*,
 mark options={solid,fill=red,draw=red}, 
 ] 
coordinates {
(5, 78) (10, 52) (15, 40) (20, 38)
};
\addlegendentry{$\AGDMF$}

\addplot [ 
 color=green!50!black,  
 %dashed,
%smooth,
 line width=0.8pt, 
 mark size=1.1pt, 
 mark=square*,
 mark options={solid,fill=green!50!black,draw=green!50!black}, 
 ] 
coordinates {
(5, 85) (10, 48)  (15, 38) (20, 30)

};
\addlegendentry{ASGD}

\addplot [ 
 color=cyan!80!black,  
% dashed,
 smooth,
 line width=0.8pt, 
 mark size=1.1pt, 
 mark=*,
 mark options={solid,fill=cyan!80!black,draw=cyan!80!black}, 
 ]  coordinates {
(5, 120) (10, 68) (15, 60) (20, 56)
};
\addlegendentry{DSGD}

\addplot [ 
 color=magenta!80!black,  
 smooth,
 line width=0.8pt, 
 mark size=1.8pt, 
 mark=star,
 %mark options={fill=cyan!50!black}, 
 ]  coordinates {
(5,100) (10, 65) (15, 58) (20, 56)
};
\addlegendentry{AD-ADMM}
{font=\fontsize{4}{5}\selectfont}

\end{axis}
\end{tikzpicture}
  \caption{(a) NF Subset}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}[b]{0.5\linewidth}
  \centering
  \begin{tikzpicture}
  \begin{axis}[ 
	width=\textwidth,
	height=\textwidth,
   compat=newest, 
   xmajorgrids,
   ymajorgrids,
   xmin=3, xmax=22,
     ymin=50, 
     ymax=350,
    %xtick={0.,50, 100, 150,200},
    %ytick={0.8, 0.9, 1, 1.1, 1.2},
   xlabel=\text{\small Number of Cores},
    ylabel=\text{\small Time Per Epoch (s)},
    legend style={font=\tiny},
%extra x ticks={120,205.2,158.4,169.5},
%extra x tick labels={\color{red} \footnotesize  \textbf{Async}, \color{green!50!black} \footnotesize  \textbf{ASGD},  \color{cyan!80!black} \footnotesize  \textbf{DSGD}, \color{magenta!80!black} \footnotesize  \textbf{AsyncWithDelay},},
%extra x tick style={grid=major, tick label style={rotate=90,anchor=west}},
  ]  

\addplot [ 
 color=red,  
%smooth,
 line width=0.8pt, 
 mark size=1.9pt, 
 mark=diamond*,
 mark options={solid,fill=red,draw=red}, 
 ]  coordinates {
(5, 200)(10, 120)(15, 100)(20, 92)
};
\addlegendentry{$\AGDMF$}



\addplot [ 
 color=green!50!black,  
 %dashed,
%smooth,
 line width=0.8pt, 
 mark size=1.1pt, 
 mark=square*,
 mark options={solid,fill=green!50!black,draw=green!50!black}, 
 ] coordinates {
(5, 230) (10, 130) (15, 100) (20, 60)
};
\addlegendentry{ASGD}

\addplot [ 
 color=cyan!80!black,  
% dashed,
 smooth,
 line width=0.8pt, 
 mark size=1.1pt, 
 mark=*,
 mark options={solid,fill=cyan!80!black,draw=cyan!80!black}, 
 ] coordinates {
 (5, 290) (10, 170) (15, 180) (20, 192)
};
\addlegendentry{DSGD}


\addplot [ 
 color=magenta!80!black,  
 smooth,
 line width=0.8pt, 
 mark size=1.8pt, 
 mark=star,
 %mark options={fill=cyan!50!black}, 
 ]  coordinates {
 (5, 270) (10, 150) (15, 146) (20, 142)
};
\addlegendentry{AD-ADMM}

{font=\fontsize{4}{5}\selectfont}

\end{axis}
\end{tikzpicture}
  \caption{(b) ML-10M}
  \label{fig:sub2}
\end{subfigure}
\caption{Total Convergence Time Vs. Number of Cores curves for ${\AGDMF}$, {\ASGD}, {\DSGD} and \texttt{AD-ADMM} on the NetFlix (a), and ML-10M (b)  Datasets.}
\label{fig:AverageTimeVsCores}
\end{figure*}

==> results.tex <==
\iffalse
\begin{figure*}[!htb]
  \centering
  \subfigure[\Webspam\ dataset]{\includegraphics[scale=0.27]{web_5_compare_train_loss.pdf}}
  \subfigure[\Epsilon\ dataset]{\includegraphics[scale=0.28]{eps_10_compare_train_loss.pdf}}
  \subfigure[\RCV\ Dataset]{\includegraphics[scale=0.28]{rcv_10_compare_train_loss.pdf}}
  \caption{Training Loss Vs Time Plot for (a) \Webspam, (b) \Epsilon\ and (c) \RCV\ Datasets}
  \label{fig:comparison_train_loss}
\end{figure*}


\begin{figure*}[!htb]
  \centering
  \subfigure[\Webspam\ dataset]{\includegraphics[scale=0.27]{web_5_compare_test_acc.pdf}}
  \subfigure[\Epsilon\ dataset]{\includegraphics[scale=0.28]{eps_10_compare_test_acc.pdf}}
  \subfigure[\RCV\ Dataset]{\includegraphics[scale=0.28]{rcv_10_compare_test_acc.pdf}}
  \caption{Test Accuracy Vs Time Plot for (a) \Webspam, (b) \Epsilon\ and (c) \RCV\ Datasets}
  \label{fig:comparison_test_accuracy}
\end{figure*}\section{Experimental Results}

\fi

We performed experiments to assess the effect of varying broadcast frequency on the performance of asynchronous methods. We were then interested in the convergence time as well as the communication overhead and the effect of increasing the number of workers.



\subsection{Effect of Varying Broadcast Frequency}

We chose varying batch sizes after which the parameter vectors were broadcasted in each worker machines. The effect of varying batch size for broadcast on the minimization of objective function on training data for \Webspam\ and \Epsilon\ datasets are shown in Figure \ref{fig:batch_performance}. As it can be observed, the broadcasting of the parameter vectors has in general a negative effect on the performance of the algorithm. In Figure \ref{fig:batch_performance}, we can notice that when the parameter was broadcasted after 1/10000 or 1/1000'th pass over the data, the minimization of the objective function is not very good, whereas  broadcasting after a larger pass over the data improves the minimization up to some point when the parameters pooling do not occur often enough. This gives a good motivation for our approach of broadcasting parameter vectors only after updating the parameter vector over one pass of the local data. 


\subsection{Evaluation of Convergence Time}

 Figure $\ref{fig:comparison_train_loss}$ and $\ref{fig:comparison_test_accuracy}$ compare the convergence results for the three methods on all datasets. The convergence results are presented in terms of minimization of the objective function in the training sub-part of the data on the  the root machine and the evolution of the test accuracy with respect to time (in seconds). As It can be observed the proposed method $\ADSVRG$ converges much faster than the other two approaches which is mainly due to the synchronization of gradients between the worker machines. The objective function is minimized considerably faster for $\ADSVRG$ than the other two methods. It can be seen that this behavior becomes more noticeable for larger datasets. For example on the \RCV\ collection, $\ADSVRG$ converges three times faster than the other methods. As an effect the test performance reached by $\ADSVRG$, at its convergence, is lower than the two others, but the difference is not significant. Also it is to be noted that the difference in the convergence speed can become even larger if some of the machines are extremely overloaded, which is generally the case in the cluster environments. 




\subsection{Communication Overhead}

\iffalse
\begin{table*}
\begin{tabular}{c cc c cc c cc}
\hline
\multirow{2}{*}{Methods} &  \multicolumn{2}{c}{\Webspam} & &  \multicolumn{2}{c}{\Epsilon} & &  \multicolumn{2}{c}{\RCV} \\ \cline{2-3}\cline{5-6}\cline{8-9}

& Number of Calls & time (sec) & & Number of Calls & time (sec)  & & Number of Calls & time (sec) \\ \hline

$\SGrad$ & 336021 & 635.44 & & 108009 & 589.9 & &  83711 & 4756.25\\ 
$\ASGrad$ & 839831 & 42.13 & & 108000 & 110.03 & &  30701 & 733.47\\ 
\textbf{$\ADSVRG$} & \textbf{33611} & \textbf{14.93} & & \textbf{12004}& \textbf{29.6} & & \textbf{8380} & \textbf{631.92}\\ \hline

\end{tabular}
\caption{Comparison of the communication overhead of all approaches on the three collections}
\label{tab:comparison_comm}
\end{table*}
%%% Speedup Result
\begin{figure*}[!h]
  \centering
  \subfigure[Loss Function Vs. Time (sec)]{\includegraphics[scale=0.278]{eps_10_speedup_train_loss.pdf}}
  \subfigure[Test Accuracy Vs. Time (sec)]{\includegraphics[scale=0.278]{eps_10_speedup_test_acc.pdf}}
  \subfigure[Speedup Vs. Number of Workers]{\includegraphics[scale=0.278]{eps_10_speedup.pdf}}
  \caption{Convergence Speedup Result for \Epsilon\ Dataset}
  \label{fig:speedup}
\end{figure*}
\fi

We also present the communication overhead incurred by each of the methods. The total communication cost for each algorithm is compared in terms of the total number of communication calls (send, receive, broadcast, gather), as well as the time spent in those calls. Since for $\SGrad$ and $\ASGrad$ methods the convergence is very slow near the tail, we compare the communication cost till the iteration when all methods achieve the same minimization of the objective function. Table \ref{tab:comparison_comm} shows the detailed results obtained for each algorithm on all datasets. It can be observed that the $\ADSVRG$ incurs the minimum communication overhead as the number of communication between the machines is very low. Most of the calls shown for $\ADSVRG$ are made during the first epoch where the gradients are synchronized. Whereas $\SGrad$ and $\ASGrad$ methods have to communicate large number of times in order to broadcast their local gradients to the master and receive the updated parameters from the master machine. Since $\SGrad$ is totally synchronous, the communication calls are blocking in nature and hence considerably slow. Whereas for $\ASGrad$ and $\ADSVRG$ the communication calls are mostly non-blocking and hence return immediately. 




\subsection{Speedup Result with Increasing Number of Workers}

Finally, we evaluate the scalability of the proposed framework with respect to the increasing number of worker machines. In this experiment, we vary the number of workers from 5 to 25, each time increasing the number of workers by 5. Figure \ref{fig:speedup} illustrates the evolution of the loss function of $\ADSVRG$ on the training set (a) as well as the test accuracy (b) with respect to time (in seconds) on the \Epsilon\ collection. Figure \ref{fig:speedup} (c) also depicts the speedup in convergence time with respect to the number of workers. In the ideal case, shown in red, when the number of workers double, the convergence time is divided by two; and hence the speedup is also doubled. From this figure, it comes out that  as the number of workers increases the $\ADSVRG$ algorithm is able to achieve a near linear speedup, which is mainly due to the fact that, it relies on very low communication between the workers which is is also shown in Table \ref{tab:comparison_comm}. On the other hand, as the number of workers increases the performance of the algorithm slightly deteriorates  


\section{Application to Matrix Factorization}
We conducted a number of experiments to empirically validate the proposed asynchronous framework on matrix factorization for recommendation where the recommendation matrix is split into $M$ rows as in Problem~\eqref{eqn:pb-split}.




We performed experiments on  Movielens-10M (ML-10M)\footnote{http://grouplens.org/datasets/movielens/} and the Netflix Collection\footnote{http://www.netflixprize.com/} that are two popular corpora in collaborative filtering. The distributed framework we considered was implemented using PySpark version 1.5.1. by connecting 7 servers with different computational power. 


Since, the focus of the paper is for shared-nothing scenario, the disparate machines do not share memory. Three of the servers had Intel Xenon E5-2640 2.60 GHz processors with 32 cores and 256 GB memory each. Two others had Intel Xenon E5-2643 3.40 GHz processors with 24 cores and 128 GB memory each and the last two ones had have Intel Xeon E5-2407 2.20GHz processors with 4 cores and 48 GB memory each. Each core of a server here corresponds to a computing node or a machine that we considered in our analysis presented in the previous sections. Even though some of the servers have identical configuration, they were running different workloads on them making the configuration similar to a real scenario case. 


One of the machines was designated as the master, and worked as the coordinator to run the experiments. This computing node dispatched the rating matrix across all the other machines. 


We stop the running algorithm on each computing node, when the difference of the loss function  between two epochs on a validation set falls below a predefined threshold, $\varepsilon$, fixed to $10^{-4}$ in our experiments. The convergence of the proposed asynchronous approach is reached when the slowest machine finishes its job, while for the synchronous {\SGO} all machines finish at the same time.


Various free parameters of {\SGO} such as learning rate ($\gamma$), regularization parameter ($\lambda$) and number of latent factors ($K$) were set following \cite{chin2015learning}, \cite{yu2014distributed}. These values as well as the datasets characteristics  are listed in Table \ref{tab:dataset_properties}.

\begin{table}[h!]
\caption{Characteristics of Datasets used in our experiments. $|\mathcal U|$ and $|\mathcal I|$ denote respectively the number of users and items.} %$\alpha$, $\lambda$ and $K$ are respectively the learning rate, the regularisation hyperparameter and the number of latent factors.}
\label{tab:dataset_properties}
\tabcolsep=0.08cm
\centering
\resizebox{0.48\textwidth}{!}{
  \begin{tabular}{ l c c c c c c c c}
  \hline
  Dataset & $|\mathcal U|$ & $|\mathcal I|$ & $\gamma$ & $\lambda$ & $K$ &  training size &  test size & sparsity\\
  \hline
  
    ML-10M & 71567 & 10681 & 0.005 & 0.05 & 100 &  9301274 & 698780 & 98.7 \%\\
  
    NetFlix (NF) & 480189 & 17770 & 0.005 & 0.05 & 40 &  99072112 & 1408395 & 99.8 \%\\

    NF-Subset & 28978 & 1821 & 0.005 & 0.05 & 40 &  3255352 & 100478 & 93.7 \%\\
    
  
  
  \hline
   
\end{tabular}
}
\end{table}

To validate the asynchronous distributed algorithm described in the previous section, we test the following four strategies:
\begin{itemize}
\item The proposed approach ({\AsyDM}) - Section \ref{sec:ADM},
\item The asynchronous distributed ADMM approach (\texttt{AD-ADMM})  \cite{Tsung15},
\item Two distributed algorithms specifically proposed for matrix factorization {\ASGD} \cite{makari2015shared} and {\DSGD} \cite{gemulla2011large} (Section \ref{sec:MF}).
\end{itemize}

\subsection{Evaluation of Convergence Time}

We begin our experiments by comparing the evolution of the loss function of Eq.~\eqref{eqn:pb} with respect to time until convergence. For synchronous methods, we plot the loss on the whole dataset divided by the total number of ratings; whereas for asynchronous methods, we plot the loss on the dataset of the slowest machine divided by the number of ratings it has. 

In addition, we plot the names of the algorithms vertically when they stop (we stopped ASGD after 20 hours on the NF dataset). Figure \ref{fig:RMSE Curve} depicts this evolution for ML-10M and NF datasets using 10 and 15 cores respectively. The synchronous and parallel distributed approaches ({\ASGD} and {\DSGD}) aggregate all the information at each epoch and thus begin to converge more sharply at the beginning. However, with these approaches, when the fastest machines finish their computations, they have to wait for slower machines; thus, they require much more time to converge than the asynchronous methods (\texttt{AD-ADMM} and {\AsyDM}). 

Finally, it comes out that {\AsyDM} converges faster than the other algorithms on both datasets. This is mainly due to the fact that {\AsyDM} does not obey to any delay mechanism as in \texttt{AD-ADMM} for instance.

\subsection{Computation and Communication Trade-off }

We performed another set of experiments aimed at measuring the effect of number of cores on performance of the proposed approach and the baselines. Figure \ref{fig:AverageTimeVsCores} depicts this effect by showing the evolution of time per epoch of the SGD method used in \texttt{AsyDM}, \texttt{ASGD}, \texttt{DSGD} and \texttt{AD-ADMM} with respect to increasing number of machines. From these experiments, it comes out that for all approaches the time per epoch of the SGD method decreases as the number of machines increases. 

But after a certain number of machines (10 in both experiments), the time per epoch of some approaches begin to be affected as the communication cost takes over the computation time. The approach that is the most affected by this is \texttt{DSGD}, as synchronizations in this case are done after each sub-epoch. We can also see that even though the per epoch speedup is best for \texttt{ASGD}, it requires a much higher number of epochs to converge as compared to \texttt{AsyDM} and \texttt{DSGD}. 

Finally, it is to be noted that Spark does not provide functionality for inter machine communication and in our implementation we saved the broadcasted parameters for the asynchronous approaches using a distributed storage (HDFS). There exist other frameworks (e.g. Message Passing Interface - MPI) that allow cores to broadcast their parameters directly to other ones and the communication overhead could be significantly reduced in this case.


\begin{figure*}[t]
%\centering

\begin{subfigure}{.5\textwidth}
  \centering
  \begin{tikzpicture}
  \begin{axis}[ 
	width=\textwidth,
	height=0.75\textwidth,
 %xmajorgrids, 
 ymajorgrids, 
yminorgrids,
   compat=newest, 
   xmin=5, xmax=21,
   ymin=110, 
   ymax=115,
  %  xtick={0.,20, 40, 60,80},
  %  ytick={0.8, 0.9, 1},
   xlabel=\text{\small time (hour.)},
    ylabel=\text{\small Loss function},
    legend style={font=\tiny},
extra x ticks={19,22,20.8,25},
extra x tick labels={\color{red} \footnotesize  \textbf{AsyDM}, \color{green!50!black} \footnotesize  \textbf{ASGD},  \color{cyan!80!black} \footnotesize  \textbf{DSGD}, \color{magenta!80!black} \footnotesize  \textbf{AD-ADMM},},
extra x tick style={grid=major, tick label style={yshift=0.45cm,rotate=90,anchor=west}},
  ]  

\addplot [ 
 color=red,  
%smooth,
 line width=0.8pt, 
 mark size=1.9pt, 
 mark=diamond*,
 mark options={solid,fill=red,draw=red}, 
 ] 
coordinates {
(0.00,321.84)(1.60,129.39)(3.19,119.13)(4.79,116.01)(6.39,114.37)(7.99,113.31)(9.58,112.56)(11.18,112.00)(12.78,111.55)(14.38,111.21)(15.97,110.92)(17.57,110.67)(19.17,110.40)
};
\addlegendentry{AsyDM}

\addplot [ 
 color=green!50!black,  
 %dashed,
%smooth,
 line width=0.8pt, 
 mark size=1.1pt, 
 mark=square*,
 mark options={solid,fill=green!50!black,draw=green!50!black}, 
 ] 
coordinates {

(0.00,322.18)(1.59,123.99)(3.18,117.48)(4.77,115.02)(6.36,113.73)(7.95,112.89)(9.54,112.28)(11.13,111.81)(12.72,111.44)(14.31,111.14)(15.90,110.90)(17.49,110.70)(19.08,110.53)(20.67,110.38)

};
\addlegendentry{ASGD}

\addplot [ 
 color=cyan!80!black,  
% dashed,
 smooth,
 line width=0.8pt, 
 mark size=1.1pt, 
 mark=*,
 mark options={solid,fill=cyan!80!black,draw=cyan!80!black}, 
 ]  coordinates {
(0.00,284.20)(2.08,120.02)(4.17,115.40)(6.25,113.59)(8.33,112.64)(10.42,111.96)(12.50,111.50)(14.58,111.15)(16.67,110.82)(18.75,110.60)(20.83,110.45)(22.92,110.41)

};
\addlegendentry{DSGD}

\addplot [ 
 color=magenta!80!black,  
 smooth,
 line width=0.8pt, 
 mark size=1.8pt, 
 mark=star,
 %mark options={fill=cyan!50!black}, 
 ]  coordinates {
(1.66,133.73)(3.31,120.46)(4.97,116.70)(6.63,114.85)(8.28,113.68)(9.94,112.88)(11.60,112.28)(13.26,111.84)(14.91,111.48)(16.57,111.19)(18.23,110.93)(19.88,110.69)(21.54,110.52)

};
\addlegendentry{AD-ADMM}
{font=\fontsize{4}{5}\selectfont}

\end{axis}
\end{tikzpicture}
  \caption{NF}
  \label{fig:sub1}
\end{subfigure}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{subfigure}{.5\textwidth}
  \centering
  \begin{tikzpicture}
  \begin{axis}[ 
	width=\textwidth,
	height=0.75\textwidth,
   compat=newest, 
   %xmajorgrids,
   ymajorgrids,
   xmin=60, xmax=325,
     ymin=95, 
     ymax=110,
    %xtick={0.,50, 100, 150,200},
    %ytick={0.8, 0.9, 1, 1.1, 1.2},
   xlabel=\text{\small time (min.)},
    ylabel=\text{\small Loss Function},
    legend style={font=\tiny},
extra x ticks={210,308.33,266.67,250.83},
extra x tick labels={\color{red} \footnotesize  \textbf{AsyDM}, \color{green!50!black} \footnotesize  \textbf{ASGD},  \color{cyan!80!black} \footnotesize  \textbf{DSGD}, \color{magenta!80!black} \footnotesize  \textbf{AD-ADMM},},
extra x tick style={grid=major, tick label style={yshift=1.5cm,rotate=90,anchor=west}},
  ]  

\addplot [ 
 color=red,  
%smooth,
 line width=0.8pt, 
 mark size=1.9pt, 
 mark=diamond*,
 mark options={solid,fill=red,draw=red}, 
 ]  coordinates {
 
(0,621.97)(15,135.34)(30,115.73)(45,109.89)(60,106.69)(75,104.63)(90,103.14)(105,102.02)(120,101.14)(135,100.43)(150,99.8)(165,99.29)(180,98.84)(195,98.39)(210,97.68)


};
\addlegendentry{AsyDM}

\addplot [ 
 color=green!50!black,  
 %dashed,
%smooth,
 line width=0.8pt, 
 mark size=1.1pt, 
 mark=square*,
 mark options={solid,fill=green!50!black,draw=green!50!black}, 
 ] coordinates {
(0.00, 627.18)(15.42, 131.33)(30.83, 116.2)(46.25, 110.49)(61.67, 107.27)(77.08, 105.15)(92.50, 103.63)(107.92, 102.48)(123.33, 101.57)(138.75, 100.82)(154.17, 100.21)(169.58, 99.68)(185.00, 99.23)(200.42, 98.84)(215.83, 98.48)(231.25, 98.18)(246.67, 97.91)(262.08, 97.67)(277.50, 97.45)(292.92, 97.26)(308.33, 97.08)
};
\addlegendentry{ASGD}

\addplot [ 
 color=cyan!80!black,  
% dashed,
 smooth,
 line width=0.8pt, 
 mark size=1.1pt, 
 mark=*,
 mark options={solid,fill=cyan!80!black,draw=cyan!80!black}, 
 ] coordinates {
(0.00,517.82)(26.67,115.25)(53.33,107.39)(80.00,104.16)(106.67,102.41)(133.33,101.23)(160.00,100.34)(186.67,99.64)(213.33,99.1)(240.00,98.55)(266.67,98.33)};
\addlegendentry{DSGD}


\addplot [ 
 color=magenta!80!black,  
 smooth,
 line width=0.8pt, 
 mark size=1.8pt, 
 mark=star,
 %mark options={fill=cyan!50!black}, 
 ]  coordinates {
(0.00,621.79)(17.92,136.25)(35.83,116.48)(53.75,110.38)(71.67,107.08)(89.58,104.93)(107.50,103.39)(125.42,102.23)(143.33,101.27)(161.25,100.5)(179.17,99.88)(197.08,99.34)(215.00,98.87)(232.92,98.42)(250.83,98.01)};
\addlegendentry{AD-ADMM}

{font=\fontsize{4}{5}\selectfont}

\end{axis}
\end{tikzpicture}
  \caption{ML-10M}
  \label{fig:sub2}
\end{subfigure}
\caption{Test RMSE curves with respect to time for {\AsyDM}, \texttt{AD-ADMM}, {\ASGD},  and {\DSGD} on NetFlix (a), and ML-10M (b) Datasets}
\label{fig:RMSE Curve}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \begin{tikzpicture}
  \begin{axis}[ 
	width=\textwidth,
	height=0.75\textwidth,
 xmajorgrids, 
 ymajorgrids, 
yminorgrids,
   compat=newest, 
   xmin=3, xmax=22,
   ymin=25, 
   ymax=100,
    xtick={5.,10, 15, 20},
    ytick={25, 50, 75, 100},
    xlabel=\text{\small Number of Cores },
    ylabel=\text{\small Time Per Epoch (sec)},
    legend style={font=\tiny},
%extra x ticks={41.8,64,60,75},
%extra x tick labels={\color{red} \footnotesize  \textbf{Async}, \color{green!50!black} \footnotesize  \textbf{ASGD},  \color{cyan!80!black} \footnotesize  \textbf{DSGD}, \color{magenta!80!black} \footnotesize  \textbf{AsyncWithDelay},},
%extra x tick style={grid=major, tick label style={rotate=90,anchor=west}},
  ]  

\addplot [ 
 color=red,  
%smooth,
 line width=0.8pt, 
 mark size=1.9pt, 
 mark=diamond*,
 mark options={solid,fill=red,draw=red}, 
 ] 
coordinates {
(5, 78) (10, 52) (15, 40) (20, 38)
};
\addlegendentry{AsyDM}

\addplot [ 
 color=green!50!black,  
 %dashed,
%smooth,
 line width=0.8pt, 
 mark size=1.1pt, 
 mark=square*,
 mark options={solid,fill=green!50!black,draw=green!50!black}, 
 ] 
coordinates {
(5, 85) (10, 48)  (15, 38) (20, 30)

};
\addlegendentry{ASGD}

\addplot [ 
 color=cyan!80!black,  
% dashed,
 smooth,
 line width=0.8pt, 
 mark size=1.1pt, 
 mark=*,
 mark options={solid,fill=cyan!80!black,draw=cyan!80!black}, 
 ]  coordinates {
(5, 120) (10, 68) (15, 60) (20, 56)
};
\addlegendentry{DSGD}

\addplot [ 
 color=magenta!80!black,  
 smooth,
 line width=0.8pt, 
 mark size=1.8pt, 
 mark=star,
 %mark options={fill=cyan!50!black}, 
 ]  coordinates {
(5,100) (10, 65) (15, 58) (20, 56)
};
\addlegendentry{AD-ADMM}
{font=\fontsize{4}{5}\selectfont}

\end{axis}
\end{tikzpicture}
  \caption{NF Subset}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \begin{tikzpicture}
  \begin{axis}[ 
	width=\textwidth,
	height=0.75\textwidth,
   compat=newest, 
   xmajorgrids,
   ymajorgrids,
   xmin=3, xmax=22,
     ymin=50, 
     ymax=350,
    %xtick={0.,50, 100, 150,200},
    %ytick={0.8, 0.9, 1, 1.1, 1.2},
   xlabel=\text{\small Number of Cores},
    ylabel=\text{\small Time Per Epoch (s)},
    legend style={font=\tiny},
%extra x ticks={120,205.2,158.4,169.5},
%extra x tick labels={\color{red} \footnotesize  \textbf{Async}, \color{green!50!black} \footnotesize  \textbf{ASGD},  \color{cyan!80!black} \footnotesize  \textbf{DSGD}, \color{magenta!80!black} \footnotesize  \textbf{AsyncWithDelay},},
%extra x tick style={grid=major, tick label style={rotate=90,anchor=west}},
  ]  

\addplot [ 
 color=red,  
%smooth,
 line width=0.8pt, 
 mark size=1.9pt, 
 mark=diamond*,
 mark options={solid,fill=red,draw=red}, 
 ]  coordinates {
(5, 200)(10, 120)(15, 100)(20, 92)
};
\addlegendentry{AsyDM}



\addplot [ 
 color=green!50!black,  
 %dashed,
%smooth,
 line width=0.8pt, 
 mark size=1.1pt, 
 mark=square*,
 mark options={solid,fill=green!50!black,draw=green!50!black}, 
 ] coordinates {
(5, 230) (10, 130) (15, 100) (20, 60)
};
\addlegendentry{ASGD}

\addplot [ 
 color=cyan!80!black,  
% dashed,
 smooth,
 line width=0.8pt, 
 mark size=1.1pt, 
 mark=*,
 mark options={solid,fill=cyan!80!black,draw=cyan!80!black}, 
 ] coordinates {
 (5, 290) (10, 170) (15, 180) (20, 192)
};
\addlegendentry{DSGD}


\addplot [ 
 color=magenta!80!black,  
 smooth,
 line width=0.8pt, 
 mark size=1.8pt, 
 mark=star,
 %mark options={fill=cyan!50!black}, 
 ]  coordinates {
 (5, 270) (10, 150) (15, 146) (20, 142)
};
\addlegendentry{AD-ADMM}

{font=\fontsize{4}{5}\selectfont}

\end{axis}
\end{tikzpicture}
  \caption{ML-10M}
  \label{fig:sub2}
\end{subfigure}
\caption{Total Convergence Time Vs. Number of Cores curves for {\AsyDM}, {\ASGD}, {\DSGD} and \texttt{AD-ADMM} on the NetFlix (a), and ML-10M (b)  Datasets.}
\label{fig:AverageTimeVsCores}
\end{figure*}
